Non-verbal Perception of Room Acoustics using Multi Dimensional Scaling Metho

Subjective room acoustics impressions play an important role for the performance and reception of music in concert venues and auralizations. Therefore, room acoustics since the 20th century dealt with the relationship between objective, acoustic parameters and subjective impressions of room acoustics. One common approach is to correlate acoustic measures with experts' subjective ratings of rooms as recalled from their long-term memory, and explain them using acoustical measures. Another approach is to let listeners rate auralized room acoustics on bipolar scales and find objective correlates. In this study, we present an alternative approach to characterizing the subjective impressions of room acoustics. We concolve music with binaural room impulse response measurements and utilize Multi Dimensional Scaling (MDS) to identify the perceptual dimensions of room acoustics. Results show that the perception of room acoustics has $5$ dimensions that can be explained by the (psycho-)acoustical measures echo density, fractal correlation dimension, roughness, loudness, and early decay time.

==> aps10pt4-1.rtx.tex <==
%%
%% This is file `aps10pt4-1.rtx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% revtex4-1.dtx  (with options: `10pt')
%% 
%% This file is part of the APS files in the REVTeX 4 distribution.
%% For the version number, search on the string 
%% Original version by David Carlisle
%% Modified by Arthur Ogawa (mailto:arthur_ogawa at sbcglobal dot net)
%% 
%% Copyright (c) 2009 The American Physical Society.
%% http://publish.aps.org/revtex4/
%% mailto:revtex4@aps.org
%% 
%% See the REVTeX 4 README file for restrictions and more information.
%% 
\ProvidesFile{aps10pt4-1}
[2010/02/25/18:00:00 4.1p (http://publish.aps.org/revtex4/ for documentation)]% \fileversion
\ifx\undefined\substyle@ext
\def\@tempa{%
	\endinput
	\GenericWarning{I must be read in by REVTeX! (Bailing out)}%
}%
\expandafter\else
\def\@tempa{}%
\expandafter\fi\@tempa
\class@info{RevTeX pointsize 10pt selected}%
\def\normalsize{%
	\@setfontsize\normalsize\@xpt{11.5}%
	\abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
	\belowdisplayskip \abovedisplayskip
	\abovedisplayshortskip  \abovedisplayskip
	\belowdisplayshortskip \abovedisplayskip
	\let\@listi\@listI
}%
\def\small{%
	\@setfontsize\small\@ixpt{10.5}%
	\abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
	\belowdisplayskip \abovedisplayskip
	\abovedisplayshortskip \z@ \@plus2\p@
	\belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
	\def\@listi{%
		\leftmargin\leftmargini
		\topsep 4\p@ \@plus2\p@ \@minus2\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep
	}%
}%
\def\footnotesize{%
	\@setfontsize\footnotesize\@viiipt{9.5pt}%
	\abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
	\belowdisplayskip \abovedisplayskip
	\abovedisplayshortskip \z@ \@plus\p@
	\belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
	\def\@listi{%
		\leftmargin\leftmargini
		\topsep 3\p@ \@plus\p@ \@minus\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep
	}%
}%
\def\scriptsize{%
	\@setfontsize\scriptsize\@viipt\@viiipt
}%
\def\tiny{%
	\@setfontsize\tiny\@vpt\@vipt
}%
\def\large{%
	\@setfontsize\large\@xiipt{14pt}%
}%
\def\Large{%
	\@setfontsize\Large\@xivpt{18pt}%
}%
\def\LARGE{%
	\@setfontsize\LARGE\@xviipt{22pt}%
}%
\def\huge{%
	\@setfontsize\huge\@xxpt{25pt}%
}%
\def\Huge{%
	\@setfontsize\Huge\@xxvpt{30pt}%
}%
\appdef\setup@hook{%
	\twoside@sw{%
		\oddsidemargin  -20pt
		\evensidemargin -20pt
		\marginparwidth 107pt
	}{%
		\oddsidemargin  -.25in
		\evensidemargin -.25in
		\marginparwidth 30pt
	}%
}%
\marginparsep 6pt
\topmargin -61pt
\headheight 25pt
\headsep 16pt
\topskip 10pt
\splittopskip\topskip
\footskip 30pt
\textheight = 56pc
\textwidth42.5pc
\columnsep 1.5pc
\columnseprule 0pt
\footnotesep 1pt
\skip\footins 39pt plus 4pt minus 12pt
\def\footnoterule{%
	\dimen@\skip\footins\divide\dimen@\tw@
	\kern-\dimen@\hrule width.5in\kern\dimen@
}%
\floatsep 12pt plus 2pt minus 2pt
\textfloatsep 20pt plus 2pt minus 4pt
\intextsep 12pt plus 2pt minus 2pt
\dblfloatsep 12pt plus 2pt minus 2pt
\dbltextfloatsep 20pt plus 2pt minus 4pt
\@fptop 0pt plus 1fil
\@fpsep 8pt plus 2fil
\@fpbot 0pt plus 1fil
\@dblfptop 0pt plus 1fil
\@dblfpsep 8pt plus 2fil
\@dblfpbot 0pt plus 1fil
\marginparpush 5pt
\parskip 0pt plus 1pt
\parindent 10pt
\emergencystretch8\p@
\partopsep 2pt plus 1pt minus 1pt
\leftmargini 25pt
\leftmarginii 22pt
\leftmarginiii 18.7pt
\leftmarginiv 17pt
\leftmarginv 10pt
\leftmarginvi 10pt
\def\@listI{%
	\leftmargin\leftmargini
	\parsep 4\p@ plus2\p@ minus\p@
	\topsep 8\p@ plus2\p@ minus4\p@
	\itemsep 4\p@ plus2\p@ minus\p@
}%
\labelsep 4pt
\def\@listii{%
	\leftmargin\leftmarginii
	\labelwidth\leftmarginii
	\advance\labelwidth-\labelsep
	\topsep 4\p@ plus2\p@ minus\p@
	\parsep 2\p@ plus\p@ minus\p@
	\itemsep \parsep
}%
\def\@listiii{%
	\leftmargin\leftmarginiii
	\labelwidth\leftmarginiii
	\advance\labelwidth-\labelsep
	\topsep 2\p@ plus\p@ minus\p@
	\parsep \z@
	\partopsep \p@ plus\z@ minus\p@
	\itemsep \topsep
}%
\def\@listiv{%
	\leftmargin\leftmarginiv
	\labelwidth\leftmarginiv
	\advance\labelwidth-\labelsep
}%
\def\@listv{%
	\leftmargin\leftmarginv
	\labelwidth\leftmarginv
	\advance\labelwidth-\labelsep
}%
\def\@listvi{%
	\leftmargin\leftmarginvi
	\labelwidth\leftmarginvi
	\advance\labelwidth-\labelsep
}%
\endinput
%%
%% End of file `aps10pt4-1.rtx'.
